Investigation of astrophysical phenomena in short time scales with "Pi of the Sky" apparatus

In this thesis the data analysis designed by author for the "Pi of the Sky" experiment is presented. The data analysis consists of data reduction and specific algorithms for identification of short time scale astrophysical processes. The algorithms have been tested and their efficiency has been determined and described. The "Pi of the Sky" prototype is collecting data since June 2004 and algorithms could be intensively studied and improved during over 700 nights. A few events of confirmed astrophysical origin and above 100 events in 10s time scale of unknown nature have been discovered. During the data collection period 3 Gamma Ray Bursts (out of 231) occurred in the field of view of the telescope, but no optical counterpart has been found. The upper limits for brightness of the optical counterpart have been determined. The continuous monitoring of the sky and own trigger for optical flashes allowed to determine limits on the number of GRBs without corresponding gamma-ray detection. This allowed determining limits on the ratio of emission collimation in optical and gamma bands, which is R >= 4.4. The perspectives of the full "Pi of the Sky" system has been studied and number of positive detections has been estimated on the level of ~ 2.5 events per year.

==> Dedication/dedication.tex <==
% Thesis Dedictation ---------------------------------------------------

\begin{dedication} %this creates the heading for the dedication page



\end{dedication}

% ----------------------------------------------------------------------

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../thesis"
%%% End: 


==> Results/single_flashes.tex <==
\begin{table}[htbp]
\begin{center}
\begin{tiny}
\begin{tabular}{|c|c|c|c|c|c|c| }
\hline
Date & UT Time & RA & Dec & $D_{cone}$ & $M_{max}$ & coinciding alerts / sources \\
\hline
2006.07.25 & 07:21:27 & 18h39m3.14s & -10o37'43'' & 26877.59 & 10.49 & \\ 
\hline
2006.07.20 & 07:24:02 & 18h41m8.83s & -10o43'39'' & 31842.61 & 9.78 & \\ 
\hline
2006.07.17 & 05:17:15 & 18h22m42.45s & -12o0'6'' & 25099.11 & - & \\ 
\hline
2006.07.17 & 04:48:47 & 23h56m13.09s & -23o52'6'' & 11975.36 & 10.1 & \\ 
\hline
2006.07.17 & 03:46:37 & 19h18m36.07s & -10o50'5'' & 34274.14 & 8.8 & \\ 
\hline
2006.07.17 & 00:55:35 & 12h12m16.84s & -65o13'37'' & 7597.41 & 10.7 & \\ 
\hline
2006.07.15 & 05:57:24 & 19h42m1.54s & -9o26'54'' & 37745.07 & 10.5 & \\ 
\hline
2006.07.15 & 03:01:12 & 18h24m2.21s & -11o56'53'' & 18369.61 & 10.1 & \\ 
\hline
2006.07.14 & 07:29:28 & 18h46m13.81s & -10o48'56'' & 39593.87 & 10.2 & \\ 
\hline
2006.07.10 & 04:51:00 & 20h5m44.80s & -10o8'5'' & 29063.88 & 9.04 & \\ 
\hline
2006.07.10 & 00:18:02 & 12h42m52.55s & 22o36'27'' & 6980.69 & 10.81 & <1 arcmin from NGP9 F378-0444065 - Galaxy, 1 arcmin from FIRST J124239.4+223536 - Radio-source \\ 
\hline
2006.07.03 & 08:42:04 & 1h2m50.01s & 4o29'27'' & 7380.32 & 9.76 & \\ 
\hline
2006.07.02 & 09:48:58 & 0h40m30.20s & 4o0'26'' & 6831.95 & 9.6 & \\ 
\hline
2006.07.02 & 08:15:12 & 1h42m27.20s & 9o34'42'' & 7413.05 & 10.45 & \\ 
\hline
2006.06.29 & 22:58:34 & 11h40m20.20s & 13o34'58'' & 6530.95 & 11.37 & \\ 
\hline
2006.06.29 & 22:49:16 & 11h38m18.76s & 11o50'8'' & 6492.79 & 8.05 & \\ 
\hline
2006.06.27 & 03:19:54 & 16h10m39.49s & -11o14'39'' & 14128.27 & 11.17 & \\ 
\hline
2006.06.27 & 02:24:34 & 18h4m16.33s & -8o4'15'' & 24909.05 & - & \\ 
\hline
2006.06.27 & 02:19:55 & 17h59m55.77s & -7o56'7'' & 23450.17 & - & \\ 
\hline
2006.06.26 & 03:51:28 & 16h39m3.75s & -11o40'55'' & 17908.50 & 11.11 & \\ 
\hline
2006.06.24 & 02:47:18 & 16h15m34.48s & -37o6'22'' & 13787.51 & 10.81 & \\ 
\hline
2006.06.23 & 09:13:04 & 23h41m41.95s & 0o1'38'' & 7174.30 & - & 7 arcsec from J234135.2-000145 Seyfert 1 Galaxy \\ 
\hline
2006.06.18 & 04:19:38 & 19h20m32.60s & -31o7'50'' & 22918.17 & 10.1 & \\ 
\hline
2006.06.14 & 09:48:41 & 22h17m47.85s & -6o26'54'' & 6873.38 & 9.7 & \\ 
\hline
2006.06.13 & 07:38:58 & 22h24m32.22s & -7o17'11'' & 8471.05 & 9.26 & \\ 
\hline
2006.06.12 & 07:53:49 & 22h1m6.08s & -10o47'12'' & 8405.26 & 10.5 & \\ 
\hline
2006.06.11 & 00:03:36 & 9h59m22.93s & 0o29'16'' & 6937.20 & 8.7 & 1 arcmin from [LPZ94] 279 -- Radio-source \\ 
\hline
2006.06.10 & 04:57:53 & 18h32m4.61s & -10o4'8'' & 21981.23 & 8.93 & \\ 
\hline
2006.06.08 & 07:44:44 & 17h31m54.42s & -11o2'14'' & 22001.87 & 8.5 & 2 arcmin from IRAS 17291-1057 - Infra-Red source \\ 
\hline
2006.06.08 & 06:08:36 & 17h44m25.43s & -17o24'2'' & 30564.76 & \\ 
\hline
2006.06.06 & 07:20:08 & 17h41m41.34s & -62o7'57'' & 11407.20 & \\ 
\hline
2006.06.05 & 00:57:09 & 12h15m14.43s & -20o19'19'' & 7959.37 & \\ 
\hline
2006.06.01 & 03:51:14 & 12h49m26.68s & 13o17'54'' & 10775.38 & - & 1 arcmin from FIRST J124926.0+131612 - Radio-source \\ 
\hline
2006.05.22 & 05:21:25 & 16h39m21.25s & -9o35'11'' & 29140.23 & - & \\ 
\hline
2006.05.21 & 05:06:28 & 15h38m6.76s & 12o49'19'' & 18604.53 & - & \\ 
\hline
2005.08.07 & 23:59:16 & 21h44m40s & -41\deg49' & 8444.05 & - & \\ 
\hline
2005.08.07 & 06:52:52 & 21h59m20s & -11\deg52' & 21841.07 & - & \\ 
\hline
2005.08.07 & 00:21:42 & 19h27m22s & -23\deg52' & 7833.39 & - & \\ 
\hline
2005.08.01 & 01:56:25 & 17h40m45s & +14\deg22' & 9352.06 & - & \\ 
\hline
2005.06.30 & 09:39:38 & 19h2m58s & -18\deg40' & 11783.78 & - & \\ 
\hline
2005.06.02 & 03:35:18 & 11h42m51s & +1\deg57' & 9668.98 & - & \\ 
\hline
2005.06.01 & 23:34:14 & 12h41m14s & +10\deg44' & 6888.54 & - & 1arcmin from GRDG +11 54 Galaxy \\ 
\hline
2005.06.01 & 22:54:14 & 12h2m24s & +12\deg49' & 6553.28 & - & \\ 
\hline
2005.06.01 & 03:47:30 & 11h50m11s & +1\deg28' & 9983.38 & - & \\ 
\hline
2005.06.01 & 00:19:37 & 12h56m19s & +14\deg21' & 7485.79 & - & \\ 
\hline
2005.05.31 & 22:56:15 & 12h23m32s & +11\deg49' & 6571.52 & - & J122331.1+114752 radio \\ 
\hline
2005.05.31 & 04:12:52 & 11h58m51s & -2\deg2' & 10570.86 & - & Konus 4:27:26 \\ 
\hline
2005.05.31 & 00:01:46 & 11h54m52s & +15\deg7' & 7110.83 & - & \\ 
\hline
2005.05.27 & 23:02:13 & 10h15m13s & +14\deg20' & 6570.98 & - & \\ 
\hline
2005.05.27 & 22:55:12 & 10h52m40s & +28\deg37' & 6537.24 & - & \\ 
\hline
2005.05.27 & 22:53:34 & 10h51m3s & +24\deg42' & 6530.79 & - & \\ 
\hline
2005.05.27 & 05:36:11 & 16h56m42s & -10\deg27' & 29060.33 & - & \\ 
\hline
2005.05.25 & 03:57:10 & 16h1m30s & -8\deg1' & 36600.71 & - & \\ 
\hline
2005.05.20 & 08:33:30 & 15h33m51s & -32\deg21' & 18299.27 & - & \\ 
\hline
2005.05.16 & 06:26:04 & 13h58m52s & -26\deg8' & 25026.63 & - & Konus 6:41:01 \\ 
\hline
2005.05.16 & 00:26:50 & 13h3m11s & -42\deg17' & 7888.47 & - & \\ 
\hline
2005.05.15 & 23:04:50 & 13h39m42s & -39\deg34' & 6659.66 & - & \\ 
\hline
2005.05.14 & 03:28:22 & 13h28m41s & -15\deg57' & 15960.10 & - & \\ 
\hline
2005.05.14 & 03:19:27 & 13h18m45s & -21\deg30' & 14734.27 & - & \\ 
\hline
2005.05.14 & 02:35:02 & 13h33m57s & -27\deg26' & 13338.49 & - & \\ 
\hline
2005.05.12 & 04:59:08 & 12h47m39s & +10\deg24' & 14673.83 & - & \\ 
\hline
2005.05.11 & 03:05:50 & 11h13m34s & +12\deg15' & 10060.39 & - & \\ 
\hline
2005.05.06 & 05:53:02 & 14h2m13s & +0\deg35' & 28414.20 & - & \\ 
\hline
2005.05.02 & 08:36:34 & 13h53m22s & -11\deg23' & 59060.43 & - & \\ 
\hline
2005.05.01 & 10:09:25 & 18h49m16s & +9\deg17' & 6571.82 & - & \\ 
\hline
2005.04.29 & 08:27:37 & 14h37m26s & -8\deg35' & 35516.11 & - & LEDA 1001633 \\ 
\hline
2005.04.24 & 06:24:24 & 16h48m39s & -10\deg18' & 11778.71 & - & \\ 
\hline
2005.04.01 & 06:12:52 & 11h16m47s & +6\deg59' & 26486.27 & - & GSC 00269-00778 \\ 
\hline
2005.03.30 & 04:45:08 & 11h0m3s & +14\deg38' & 19964.19 & - & \\ 
\hline
2005.02.16 & 00:32:49 & 10h0m19s & -13\deg16' & 6745.62 & - & \\ 
\hline
2005.02.15 & 08:01:54 & 10h8m17s & +13\deg10' & 23523.08 & - & \\ 
\hline
2005.02.15 & 06:51:10 & 11h6m27s & +19\deg57' & 15588.09 & - & \\ 
\hline
2005.02.15 & 04:54:47 & 11h0m10s & +6\deg16' & 17082.21 & - & \\ 
\hline
2005.02.12 & 03:24:46 & 9h45m31s & -14\deg43' & 9815.57 & - & \\ 
\hline
2005.02.04 & 07:07:33 & 9h51m46s & +12\deg19' & 12323.42 & - & \\ 
\hline
2005.01.31 & 00:35:47 & 7h0m11s & +11\deg37' & 6567.26 & - & \\ 
\hline
2005.01.28 & 07:09:05 & 6h48m39s & +13\deg23' & 17545.88 & - & \\ 
\hline
2005.01.17 & 04:01:01 & 8h49m0s & +17\deg12' & 21936.75 & - & \\ 
\hline
2005.01.10 & 00:54:15 & 5h10m31s & +13\deg40' & 6624.79 & - & \\ 
\hline
2005.01.09 & 02:23:36 & 6h58m53s & +17\deg11' & 10701.16 & - & \\ 
\hline
2005.01.09 & 01:45:03 & 6h15m2s & +18\deg45' & 7730.47 & - & \\ 
\hline
2005.01.07 & 02:52:50 & 6h2m36s & +9\deg6' & 8639.52 & - & \\ 
\hline
2005.01.03 & 06:34:48 & 7h59m55s & 18\deg0' & 10149.77 & - & \\ 
\hline
2005.01.02 & 06:41:28 & 5h59m41s & +20\deg53' & 30460.54 & - & Konus+Integral 6:27:27 \\ 
\hline
2004.12.27 & 07:22:21 & 5h48m30s & 0\deg0' & 8073.92 & - & \\ 
\hline
2004.12.27 & 03:51:03 & 4h49m40s & +19\deg58' & 11531.88 & - & \\ 
\hline
2004.12.22 & 02:22:12 & 7h7m3s & +17\deg41' & 20513.74 & - & \\ 
\hline
2004.12.20 & 02:24:46 & 5h56m24s & +3\deg10' & 8343.60 & - & \\ 
\hline
2004.12.19 & 02:46:43 & 5h3m58s & +7\deg34' & 8624.41 & - & \\ 
\hline
2004.12.18 & 05:53:37 & 5h48m38s & +12\deg26' & 11325.46 & - & \\ 
\hline
2004.12.14 & 02:29:21 & 5h32m9s & +14\deg29' & 11375.21 & - & \\ 
\hline
2004.12.13 & 05:23:02 & 5h26m40s & -1\deg16' & 9123.02 & - & \\ 
\hline
2004.12.11 & 00:47:21 & 3h13m14s & +6\deg9' & 6640.76 & - & \\ 
\hline
2004.12.04 & 07:34:46 & 5h19m21s & +14\deg34' & 7944.71 & - & \\ 
\hline
2004.12.04 & 06:28:54 & 5h5m28s & +21\deg15' & 18083.59 & - & \\ 
\hline
2004.12.04 & 02:05:22 & 3h1m51s & +5\deg57' & 7689.37 & - & galaxy [ZHG90] 0259+0545 \\ 
\hline
2004.12.02 & 05:13:41 & 4h7m24s & +20\deg27' & 35733.74 & - & \\ 
\hline
2004.12.01 & 01:28:47 & 1h34m19s & +14\deg51' & 7123.42 & - & \\ 
\hline
2004.11.30 & 04:09:42 & 3h21m4s & +19\deg1' & 15993.36 & - & \\ 
\hline
2004.11.28 & 04:27:16 & 1h27m28s & +10\deg48' & 10041.09 & - & \\ 
\hline
2004.11.28 & 03:20:15 & 3h4m44s & +5\deg42' & 9501.62 & - & \\ 
\hline
2004.11.26 & 05:58:15 & 5h10m12s & +14\deg40' & 11027.50 & - & \\ 
\hline
2004.11.24 & 07:39:33 & 6h54m30s & +18\deg49' & 7145.41 & - & \\ 
\hline
2004.11.23 & 02:39:10 & 5h14m29s & -7\deg6' & 9110.72 & - & \\ 
\hline
2004.11.19 & 00:53:08 & 3h14m50s & +3\deg20' & 7165.51 & - & \\ 
\hline
2004.11.18 & 07:53:55 & 4h22m13s & +12\deg31' & 7505.47 & - & \\ 
\hline
2004.11.18 & 01:36:09 & 3h10m22s & +3\deg12' & 8120.09 & - & \\ 
\hline
2004.11.18 & 00:25:36 & 1h30m17s & +11\deg44' & 6655.27 & - & \\ 
\hline
2004.11.17 & 03:31:17 & 2h48m36s & +11\deg13' & 13252.46 & - & \\ 
\hline
2004.11.12 & 02:51:31 & 2h27m12s & +22\deg6' & 23386.60 & - & \\ 
\hline
2004.11.11 & 04:46:43 & 2h8m7s & +10\deg13' & 16192.00 & - & \\ 
\hline
2004.11.11 & 01:57:49 & 4h3m47s & +18\deg33' & 39316.77 & - & \\ 
\hline
2004.11.06 & 06:02:58 & 3h47m24s & +10\deg22' & 12004.63 & - & \\ 
\hline
2004.11.05 & 07:49:20 & 2h34m32s & +5\deg47' & 9813.32 & - & \\ 
\hline
2004.11.03 & 01:22:40 & 0h12m32s & +0\deg49' & 7482.92 & - & Konus 1:26:43, Integral 1:27:11 \\ 
\hline
2004.11.02 & 07:14:15 & 1h23m53s & +1\deg13' & 13855.20 & - & Konus 7:27:56 \\ 
\hline
2004.11.01 & 05:49:34 & 23h47m44s & -4\deg23' & 10893.98 & - & \\ 
\hline
2004.11.01 & 05:22:28 & 23h20m39s & -5\deg43' & 10146.59 & - & \\ 
\hline
2004.10.31 & 06:15:37 & 23h24m40s & -1\deg12' & 11214.86 & - & \\ 
\hline
2004.10.30 & 05:22:06 & 0h42m54s & -29\deg30' & 9093.59 & - & \\ 
\hline
2004.10.28 & 02:56:42 & 3h34m40s & -8\deg15' & 11525.31 & - & \\ 
\hline
2004.10.24 & 03:40:00 & 0h36m31s & -5\deg10' & 11388.33 & - & Radio-source Cul 0034-054 \\ 
\hline
2004.10.21 & 02:36:00 & 1h2m16s & -4\deg17' & 11101.45 & - & \\ 
\hline
2004.10.11 & 07:37:09 & 3h12m8s & +10\deg39' & 8485.28 & - & \\ 
\hline
2004.10.11 & 06:15:13 & 2h54m57s & +18\deg16' & 13331.99 & - & \\ 
\hline
2004.10.05 & 04:18:40 & 1h24m4s & +14\deg17' & 41060.68 & - & \\ 
\hline
2004.10.02 & 02:20:50 & 23h5m26s & +12\deg36' & 13430.52 & - & \\ 
\hline
2004.10.01 & 04:09:12 & 21h46m26s & -8\deg18' & 11642.37 & - & \\ 
\hline
2004.09.30 & 00:49:38 & 23h19m50s & -2\deg36' & 8307.80 & - & \\ 
\hline
2004.09.27 & 04:20:55 & 3h29m33s & +14\deg8' & 12965.21 & - & \\ 
\hline
2004.09.17 & 03:50:25 & 23h42m55s & +31\deg44' & 20126.16 & - & \\ 
\hline
2004.09.13 & 03:33:52 & 0h14m45s & +2\deg50' & 40744.17 & - & \\ 
\hline
\end{tabular}
\end{tiny}
\hfill
\caption{Optical flashes indentified by the on-line algorithm requiring
coincindece of flash on 2 cameras. These flashes were observed on single 10s
exposure}
\label{all_singles}
\end{center}
\end{table}

